Analysis of Phylogeny Tracking Algorithms for Serial and Multiprocess Applications

Since the advent of modern bioinformatics, the challenging, multifaceted problem of reconstructing phylogenetic history from biological sequences has hatched perennial statistical and algorithmic innovation. Studies of the phylogenetic dynamics of digital, agent-based evolutionary models motivate a peculiar converse question: how to best engineer tracking to facilitate fast, accurate, and memory-efficient lineage reconstructions? Here, we formally describe procedures for phylogenetic analysis in both serial and distributed computing scenarios. With respect to the former, we demonstrate reference-counting-based pruning of extinct lineages. For the latter, we introduce a trie-based phylogenetic reconstruction approach for "hereditary stratigraphy" genome annotations. This process allows phylogenetic relationships between genomes to be inferred by comparing their similarities, akin to reconstruction of natural history from biological DNA sequences. Phylogenetic analysis capabilities significantly advance distributed agent-based simulations as a tool for evolutionary research, and also benefit application-oriented evolutionary computing. Such tracing could extend also to other digital artifacts that proliferate through replication, like digital media and computer viruses.

==> Dockerfile <==
FROM mmore500/docker-texlive-full:sha-ea45eb5

SHELL ["/bin/bash", "-c"]

# Prevent interactive time zone config.
# adapted from https://askubuntu.com/a/1013396
ENV DEBIAN_FRONTEND=noninteractive

RUN \
  echo 'Acquire::http::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::ftp::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::Retries "100";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo "buffed apt-get resiliency"

RUN \
  find /etc/apt -type f -name '*.list' -exec sed -i 's/\(^deb.*-backports.*\)/#\1/; s/\(^deb.*-updates.*\)/#\1/; s/\(^deb.*-proposed.*\)/#\1/; s/\(^deb.*-security.*\)/#\1/' {} + \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "removed -backports, -updates, -proposed, -security repositories"

# magic to fix java installation conflict in subsequent apt install
# see https://github.com/geerlingguy/ansible-role-java/issues/64
RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    man \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  mkdir /usr/share/man/man1/

RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    bibtool \
    git \
    make \
    moreutils \
    nodejs \
    pcregrep \
    pdftk \
    tree \
    && \
  rm -rf /var/lib/apt/lists/*

CMD ["bash"]


==> Makefile <==
SHELL=/bin/bash

# get the basename of the containing directory
# this will be used to name othe output document
BUILD_DIR := $(shell basename $(abspath $(dir $(lastword $(MAKEFILE_LIST)))/..))

DRAFT_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}-draft.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

RELEASE_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

all: ${BUILD_DIR}-draft.pdf

draft: ${BUILD_DIR}-draft.pdf ${BUILD_DIR}-manuscript-draft.pdf ${BUILD_DIR}-supplement-draft.pdf ${BUILD_DIR}-draft.tex

release: ${BUILD_DIR}.pdf ${BUILD_DIR}-manuscript.pdf ${BUILD_DIR}-supplement.pdf ${BUILD_DIR}.tex

quick:
	pdflatex main.tex

${BUILD_DIR}.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR} \
    -pdflatex="pdflatex -interaction=nonstopmode" main.tex

${BUILD_DIR}.tex: main.tex
	./script/latexpand.pl main.tex > ${BUILD_DIR}.tex

${BUILD_DIR}-manuscript.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat 1-$$(( $(RELEASE_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript.pdf

${BUILD_DIR}-supplement.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat $(RELEASE_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement.pdf

${BUILD_DIR}-draft.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR}-draft \
    -pdflatex="pdflatex -interaction=nonstopmode" draft.tex

${BUILD_DIR}-draft.tex: main.tex
	./script/latexpand.pl draft.tex > ${BUILD_DIR}-draft.tex

${BUILD_DIR}-manuscript-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat 1-$$(( $(DRAFT_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript-draft.pdf

${BUILD_DIR}-supplement-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat $(DRAFT_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement-draft.pdf

fresh: cleaner all

clean:
	rm -f ${BUILD_DIR}.pdf
	rm -f ${BUILD_DIR}.tex
	rm -f ${BUILD_DIR}-draft.pdf
	rm -f ${BUILD_DIR}-draft.tex
	rm -f ${BUILD_DIR}-manuscript.pdf
	rm -f ${BUILD_DIR}-manuscript-draft.pdf
	rm -f ${BUILD_DIR}-supplement.pdf
	rm -f ${BUILD_DIR}-supplement-draft.pdf

sview:
	xdg-open ${BUILD_DIR}-draft.pdf 2>/dev/null

cleaner: clean
	latexmk -CA
	# remove auxillary files, excepting .tex and .bib files
	find . -type f -name ${BUILD_DIR}"*" ! -name '*.tex' ! -name '*.bib' -delete
	rm -rf *.bbl *.blg *.aux

.PHONY: draft release clean sview cleaner fresh quick


==> alg/curbed-recency-proportional-resolution-algo-enum-retained-ranks.tex <==
% TODO: missing pseudocode
\begin{algorithm}
\caption{Curbed Recency-proportional Resolution Stratum Enumeration}
\label{alg:curbed-recency-proportional-algo-enum-retained-ranks}
\begin{algorithmic}[1]
\State{Define $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
\While{$\#P > 1$}
\State{Find an optimal partition tree $T_{C^\prime}$ }
\State{Update $P := (P{\setminus} C^\prime) \cup \{ \bigcup_{t\in C^\prime} t \}$}
\State{Update $T := T \cup \{ \bigcup_{t\in\tau} t : \tau\in T_{C^\prime}{\setminus}
\mathcal{L}(T_{C^\prime})\}$}
\EndWhile
\Return $T$
\end{algorithmic}
\end{algorithm}


==> alg/curbed-recency-proportional-resolution-algo-gen-drop-ranks.tex <==
% TODO: missing pseudocode
\begin{algorithm}
\caption{Curbed Recency-proportional Resolution Stratum Discard Generator}
\label{alg:curbed-recency-proportional-algo-gen-drop-ranks}
\begin{algorithmic}[1]
\State{Define $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
\While{$\#P > 1$}
\State{Find an optimal partition tree $T_{C^\prime}$ }
\State{Update $P := (P{\setminus} C^\prime) \cup \{ \bigcup_{t\in C^\prime} t \}$}
\State{Update $T := T \cup \{ \bigcup_{t\in\tau} t : \tau\in T_{C^\prime}{\setminus}
\mathcal{L}(T_{C^\prime})\}$}
\EndWhile
\Return $T$
\end{algorithmic}
\end{algorithm}


==> alg/curbed-recency-proportional-resolution-algo-pred-keep-rank.tex <==
% TODO: missing pseudocode
\begin{algorithm}
\caption{Curbed Recency-proportional Resolution Stratum Retention Predicate}
\label{alg:curbed-recency-proportional-algo-pred-keep-rank}
\begin{algorithmic}[1]
\State{Define $P:=T:=\{ \{1\},\ldots,\{d\}$\}}
\While{$\#P > 1$}
\State{Find an optimal partition tree $T_{C^\prime}$ }
\State{Update $P := (P{\setminus} C^\prime) \cup \{ \bigcup_{t\in C^\prime} t \}$}
\State{Update $T := T \cup \{ \bigcup_{t\in\tau} t : \tau\in T_{C^\prime}{\setminus}
\mathcal{L}(T_{C^\prime})\}$}
\EndWhile
\Return $T$
\end{algorithmic}
\end{algorithm}


==> alg/depth-proportional-resolution-algo-enum-retained-ranks.tex <==
\begin{algorithm}
\caption{Depth-proportional Resolution Stratum Enumeration}
\label{alg:depth-proportional-resolution-algo-enum-retained-ranks}
\begin{algorithmic}[1]
    \Require{ $\texttt{n}$ -- the number of strata deposited }
    \Require{ $\texttt{r}$ -- the fixed resolution desired }
    \Ensure{ array of retained strata }

    \State $\texttt{uncertainty} \gets (\text{largest integral power of two} \le \frac{n}{r + 1}) \lor 1$
    \State $\texttt{arr} \gets \text{empty array of length } \frac{n}{\texttt{uncertainty}} + 1$

    \For{$i = 0$ \textbf{to} $\texttt{n} - 1$ \textbf{step} $\text{uncertainty}$}
        \State $\texttt{arr} [$i$] \gets i$
    \EndFor
    \State $\texttt{last\_rank} \gets \texttt{n} - 1$
    \If{$\texttt{last\_rank} > 0$ \textbf{and} $\texttt{last\_rank} \bmod \texttt{uncertainty} \neq 0$}
        \State $\texttt{\texttt{last\_rank}} [$i$] \gets \texttt{last\_rank}$
    \EndIf
\end{algorithmic}
\end{algorithm}


==> alg/depth-proportional-resolution-algo-gen-drop-ranks.tex <==
\begin{algorithm}
\caption{Depth-proportional Resolution Discard Generator}
\label{alg:depth-proportional-resolution-algo-gen-drop-ranks}
\begin{algorithmic}[1]
    \Require{ $\texttt{n}$ -- the number of strata deposited }
    \Require{ $\texttt{r}$ -- the fixed resolution desired }
    \Ensure{ array of dropped strata }

    \State $\texttt{curr\_uncertainty} \gets (\text{largest integral power of two} \le \frac{n}{r + 2}) \lor 1$
    \State $\texttt{prev\_uncertainty} \gets (\text{largest integral power of two} \le \frac{n}{r + 1}) \lor 1$
    \State $\texttt{arr} \gets \text{empty array of length } \frac{n}{\texttt{uncertainty}} + 1$

    \If{$\texttt{curr\_uncertainty} \neq \texttt{prev\_uncertainty}$}
        \For{$i = \texttt{prev\_uncertainty}$ \textbf{to} $\texttt{n} - 2$ \textbf{step} $\text{curr\_uncertainty}$}
            \State $\texttt{arr} [$i$] \gets i$
        \EndFor
    \EndIf
    \If{$\texttt{n} - 2 \bmod \texttt{curr\_uncertainty} \neq 0$}
        \State $\texttt{\texttt{last\_rank}} [\texttt{n} - 2] \gets \texttt{n} - 2$
    \EndIf
\end{algorithmic}
\end{algorithm}


==> alg/depth-proportional-resolution-algo-pred-keep-rank.tex <==
\begin{algorithm}
\caption{Depth-proportional Resolution Stratum Retention Predicate}
\label{alg:depth-proportional-resolution-algo-pred-keep-rank}
% STUB ALGORITHM
\end{algorithm}


==> alg/fixed-resolution-algo-enum-retained-ranks.tex <==
\begin{algorithm}
\caption{Fixed Resolution Stratum Enumeration}
\label{alg:fixed-resolution-enum-retained-rans}
% STUB ALGORITHM
% \begin{algorithmic}[1]
%     \Require{$\texttt{n}$ -- the number of strata deposited}
%     \Require{$\texttt{r}$ -- the fixed resolution desired}
%     \For{$i = 0$ \textbf{to} $\texttt{n} - 1$ \textbf{step} $\texttt{r}$}
%         \State{ \textbf{yield} $i$ }
%     \EndFor
%     \State{ $\texttt{last\_rank} \gets \texttt{n} - 1$ }
%     \If{$\texttt{last\_rank} > 0$ \textbf{and} $(\texttt{last\_rank} \mod \texttt{r}) \neq 0$}
%         \State{ \textbf{yield} $\texttt{last\_rank}$ }
%     \EndIf
% \end{algorithmic}
\end{algorithm}


==> alg/fixed-resolution-algo-gen-drop-ranks.tex <==
\begin{algorithm}
\caption{Fixed Resolution Stratum Enumeration}
\label{alg:fixed-resolution-enum-retained-rans}
% STUB ALGORITHM
\end{algorithm}


==> alg/fixed-resolution-algo-pred-keep-rank.tex <==
\begin{algorithm}
\caption{Fixed Resolution Stratum Retention Predicate}
\label{alg:fixed-resolution-pred-keep-rank}
% STUB ALGORITHM
\end{algorithm}


==> alg/geom-seq-nth-root-algo-enum-retained-ranks.tex <==
\begin{algorithm}
\caption{Geometric Sequence $n$th Root Stratum Enumeration}
\label{alg:geom-seq-nth-root-enum-retained-ranks}
\begin{algorithmic}
    \Require{ $\texttt{n}$ -- the number of strata deposited }
    \Require{ $\texttt{p}$ -- the interspersal  }
    \Require{ $\texttt{d}$ -- the degree } 
    \Ensure{ set of retained strata }
\end{algorithmic}

\begin{algorithmic}[1]
    \State $\texttt{set} \gets {0, n - 1}$

    \For{$p = 1$ \textbf{to} $\texttt{d} + 1$}
        \State $\texttt{r} \gets n^{\frac{p}{d}}$

        \State $\texttt{k} \gets \text{largest integral power of two} \le \max \{\frac{r}{p}, 1 \}$ % retained_ranks_sep

        \State $\texttt{c} \gets \max \{n - \ceil{r + \frac{r}{p}}, 0\}$
        \State $\texttt{a} \gets \texttt{c} - (\texttt{c} \bmod -\texttt{k})$

        \State $\texttt{set} \gets \texttt{set} \cup \{\texttt{a}, \texttt{a} + \texttt{k}, \texttt{a} + 2\texttt{k}, {a} + 3\texttt{k}, \dots, n\}$
    \EndFor
\end{algorithmic}
\end{algorithm}


==> alg/geom-seq-nth-root-algo-gen-drop-ranks.tex <==
\begin{algorithm}
\caption{Geometric Sequence $n$th Root Stratum Discard Generator}
\label{alg:geom-seq-nth-root-gen-drop-ranks}
% STUB ALGORITHM
\end{algorithm}


==> alg/geom-seq-nth-root-algo-pred-keep-rank.tex <==
% TODO: missing pseudocode
\begin{algorithm}
\caption{Geometric Sequence $n$th Root Stratum Retention Predicate}
\label{alg:geom-seq-nth-root-algo-pred-keep-rank}
% STUB ALGORITHM
\end{algorithm}


==> alg/recency-proportional-resolution-algo-enum-retained-ranks.tex <==
\begin{algorithm}
\caption{Geometric Sequence $n$th Root Stratum Enumeration}
\label{alg:recency-proportional-resolution-algo-enum-retained-ranks}
% STUB ALGORITHM
\end{algorithm}


==> alg/recency-proportional-resolution-algo-gen-drop-ranks.tex <==
\begin{algorithm}
\caption{Recency-proportional Resolution Stratum Discard Generator}
\label{alg:recency-proportional-algo-gen-drop-ranks}
\begin{algorithmic}
    \Require{ $\texttt{n}$ -- the number of strata deposited }
    \Require{ $\texttt{r}$ -- the fixed resolution desired }
    \Ensure{ array of dropped strata }

    \Procedure{NumberToCondemn}{$\texttt{n}, \texttt{r}$}
        \If{$(\texttt{n} \bmod 2 = 1) \lor (\texttt{n} < 2 \cdot \texttt{r} + 1)$}
            \Return $0$
        \Else
            \Return $1 + \Call{NumberToCondemn}{$\texttt{n} / 2$, \texttt{r}}$
        \EndIf
    \EndProcedure

    \State $\texttt{num\_to\_condemn} \gets \Call{NumberToCondemn}{\texttt{n}, \texttt{r}}$
    \State $\texttt{arr} \gets \text{empty array of length num\_to\_condemn}$

    \For{$i = 0$ \textbf{to} $\texttt{num\_to\_condemn} - 1$}
        \State $\texttt{arr} [$i$] \gets \texttt{n} - 2^{i} \cdot (2 \texttt{r} + 1)$
    \EndFor
\end{algorithmic}
\end{algorithm}


==> alg/recency-proportional-resolution-algo-pred-keep-rank.tex <==
\begin{algorithm}
\caption{Recency-proportional Resolution Stratum Retention Predicate}
\label{alg:recency-proportional-resolution-algo-pred-keep-rank}
% STUB ALGORITHM
\end{algorithm}


==> draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> fig/retention-policies.tex <==
\input{lib/dissertationelse.tex}
\input{lib/dissertationonly.tex}

\begin{figure*}
  \centering
  \footnotesize
  \begin{tabular}{m{0.07\textwidth}@{}|c@{}|c@{\hskip 0.01\textwidth}|m{0.14\textwidth}}
%-------------------------------------------------------------------------------
\hspace{-1ex}Policy&Lower-Resolution Parameterization&Higher-Resolution Parameterization&\makecell[c]{Properties}\\\hline
%-------------------------------------------------------------------------------
    \rotatebox{90}{\textbf{Fixed Resolution}}
  &
    \makecell{
      \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/fixed_resolution=512+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/fixed_resolution=128+num_layers=1024+stratum_retention_predicate=fixed-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $\mathcal{O}(n)$\\
    \bf{MRCA Uncertainty}\\
    $\mathcal{O}(1)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=10em,
      rotate=90,
    }{
      \centering
      \textbf{Depth-Proportional\\Resolution}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $\mathcal{O}(1)$\\
    \bf{MRCA Uncertainty}\\
    $\mathcal{O}(n)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $n$ is gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
  \adjustbox{
    minipage=10em,
    rotate=90,
  }{
    \centering
    \textbf{Recency-proportional\\Resolution}
    \par
  }
  &
  \makecell{
    \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=0+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell{
    \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_mrca_recency_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=recency-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
  }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $\mathcal{O}(\log(n))$\\
    \bf{MRCA Uncertainty}\\
    $\mathcal{O}(m)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $m$ is gens since MRCA and $n$ is total gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=10em,
      rotate=90,
    }{
      \centering
      \textbf{Geometric Sequence\\$n$th Root}
      \par
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
    \makecell{
      \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $\mathcal{O}(1)$\\
    \bf{MRCA Uncertainty}\\
    $\mathcal{O}(n^{1/a} \times m)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
    where $m$ is gens since MRCA, $a$ is a user-chosen constant, and $n$ is total gens elapsed.
  }\\\hline
%-------------------------------------------------------------------------------
    \adjustbox{
      minipage=10em,
    rotate=90,
    }{
      \centering
      \textbf{Curbed Recency-proportional Resolution}
      \par
    }
  &
    %TODO generate this graphic
    \makecell{
      \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=1+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  %TODO generate this graphic
    \makecell{
      \includegraphics[valign=t,width=0.3\textwidth]{hereditary-stratigraph-concept/tex/submodules/hereditary-stratigraph-concept-binder/binder/retention-policies/teeplots/guaranteed_depth_proportional_resolution=4+num_layers=1024+stratum_retention_predicate=tapered-depth-proportional-resolution+viz=tweaked-stratum-retention-drip-plot+ext=}
    }
  &
  \makecell[{{p{0.14\textwidth}}}]{
  \centering
    \bf{Space Complexity}\\
    $\mathcal{O}(1)$\\
    \bf{MRCA Uncertainty}\\
    $\mathcal{O}(n^{1/a} \times m)$
  }
  \makecell[{{p{0.14\textwidth}}}]{
  \raggedright
   where $m$ is gens since MRCA, $a$ is a user-chosen constant, and $n$ is total gens elapsed.
  }


  \end{tabular}
  \caption{
  Comparison of streaming curation policy algorithms.
  Policy visualizations show retained strata in black.
  Time progresses along the $y$-axis from top to bottom.
  New strata are introduced along the diagonal and then ``drip'' downward as a vertical line until eliminated.
  The set of retained strata present within a column at a particular generation $g$ can be read as intersections of retained vertical lines with a horizontal line with intercept $g$.
  Policy visualizations are provided for two contrastive parameterizations for each policy algorithm.
  }
  \label{fig:retention-policies}
\end{figure*}


==> lib/dissertationelse.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationelse}[2]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
#1
\else
#2
\fi
}


==> lib/dissertationexclude.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> lib/dissertationonly.tex <==
% \pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\providecommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
}


==> lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> text/acknowledgement.tex <==
\section*{Acknowledgment}

This material is based upon work supported by the Eric and Wendy Schmidt AI in Science Postdoctoral Fellowship, a Schmidt Futures program.


==> text/body/annotation-algorithms.tex <==
\section{Streaming Curation Algorithms} \label{sec:annotation-algorithms}

\input{fig/retention-policies.tex}

This section collects specification and validation of five proposed streaming curation algorithms.
These algorithms operate online on a rolling stream of incoming observations to maintain a representative subsample of retained observations.
Streaming curation algorithms differ in the growth rate allowed for the curated observation collection and with respect to relative prioritization of retaining recent observations compared to older observations.

% For each surveyed algorithm, we present
% \begin{itemize}
% \item narration of retention policy algorithm strategy,
% \item retention policy algorithm extant record size order of growth (i.e., the scaling relationship between record depth and curated collection size),
% \item resolution guarantees (i.e., bounds on gap size between retained observations),
% \item instructions to enumerate time points retained within the curated subsample for any record depth,
% \item validation of policy algorithm self-consistency (i.e., that preceding record depths retain all observation time points required at later record depths),
% \item an algorithm for policy enactment (i.e., what observations to drop at each successive depth), and
% \item reflection of likely use case scenarios.
% \end{itemize}

We introduce the following five curation policy algorithms,
\begin{itemize}
\item Fixed-Resolution (FR) Policy Algorithm (Section \ref{sec:fixed-resolution-algo}),
\item Depth-Proportional Resolution (DPR) Policy Algorithm (Section \ref{sec:depth-proportional-resolution-algo}),
\item Recency-Proportional Resolution (RPR) Policy Algorithm (Section \ref{sec:recency-proportional-resolution-algo}),
\item Geometric Seqpence $n$th Root(GSNR) Policy Algorithm (Section \ref{sec:geom-seq-nth-root-algo}), and
\item Curbed Recency-Proportional Resolution (CRPR) Policy Algorithm (Section \ref{sec:curbed-recency-proportional-resolution-algo}).
\end{itemize}
The accomanying \texttt{hstrat} library provides reference implementations for all five.
Figure \ref{fig:retention-policies} compares retention patterns induced by each algorithm and recaps each policy algorithm's principal properties.
FR and DPR follow even curation prioritization while RPR, GSNR, and CRPR follow recency-proportional curation prioritization.
Recency-proportional techniques are of particular interest due to predictions from coalescence theory \citep{nordborgCoalescentTheory2019, berestyckiRecentProgressCoalescent2009}, which suggest that in most cases there will be more lineage divergences in recent time points.
Thus, prioritizing recent data should often improve the accuracy of subsequent data analysis.
% should we justify recency-proporitonal here?
% ELD: Added it
Collection size grows the most aggressively under FR as $\mathcal{O}(n)$.
RPR reduces collection size growth to $\mathcal{O}(\log n)$.
The remaining algorithms enforce a fixed cap on curated collection size.
Note that GSNR and CRPR exhibit identical asymptotic properties.
We include both, as CRPR is an engineered extension of GSNR that improves the efficacy of available space usage during initial shallow record depth.

Appropriate algorithm choice will depend on use case scenario.
Relevant criteria to consider include
\begin{itemize}
  \item uncertainty and magnitude of upper bounds on record depth, if any,
  \item available storage capacity,
  \item relative importance of recent and ancient observations, and
  \item any hard record quality requirements (i.e., maximum acceptable gap size).
\end{itemize}

In a real-time scenario, record depth bounds would be considered in terms of upper bounds on chronological duration of record collection and the real-time sampling rate of observations.

\input{text/body/annotation-algorithms/fixed-resolution-algo.tex}

\input{text/body/annotation-algorithms/depth-proportional-resolution-algo.tex}

\input{text/body/annotation-algorithms/recency-proportional-resolution-algo.tex}

\input{text/body/annotation-algorithms/geom-seq-nth-root-algo.tex}

\input{text/body/annotation-algorithms/curbed-recency-proportional-resolution-algo.tex}


==> text/body/annotation-algorithms/curbed-recency-proportional-resolution-algo.tex <==
\subsection{Curbed Recency-proportional Resolution (CRPR) Policy Algorithm}
\label{sec:curbed-recency-proportional-resolution-algo}

The curbed recency-proportional resolution (CRPR) policy algorithm exists to enhance in-practice utility of recency-proportional resolution.
This policy algorithm combines the geometric sequence $n$th root (GSNR) and recency-proportional resolution (RPR) algorithms to harness the strengths of both.
Figure \ref{fig:retention-policies} includes a time-lapse of the extant record under the CRPR policy algorithm.

The GSNR algorithm sustains best-effort recency-proportional resolution to asymptotic limits, but distributes retained observations less effectively than RPR in earlier periods.
This can result in higher worst-case recency-proportional gap size than necessary.
However, RPR only makes use of available storage space up to the retention density of its parameterized resolution.
Parameterizing low resolution to provide support for long historical depths would cause majorities of available storage space to go unused earlier on.
Nevertheless, ultimately at even the lowest possible parameterized resolution, extant record size will eventually outgrow any size cap under RPR.

The CRPR policy algorithm delivers the best of both worlds: full, effective storage space use of high-resolution parameterized RPR policy plus the graceful, indefinite tail support of GSNR policy.
It does this, actually, by stitching these two policy algorithms together.
In fact, CRPR stitches successively degrading RPR parameterizations together and then, once the lowest-resolution RPR policy would exceed available space, it switches to GSNR.
The CRPR policy algorithm itself provides $\mathcal{O}(1)$ extant record size order of growth, and is parameterized by a desired upper bound $m$ on retained observation count.
Support is provided for $m \geq 8$.

The CRPR policy switches from RPR to GSNR at time point,
\begin{align*}
n = \left\lfloor \frac{2^{\lfloor m/3 \rfloor}}{2} \right\rfloor
\end{align*}

with the delegated-to GSNR policy algorithm permanently parameterized to degree:
\begin{align*}
a = \max \left(
  \left\lfloor \frac{m - 2}{6} \right\rfloor,
  1
\right).
\end{align*}

At preceding time points $n$, RPR policy is parameterized to resolution
\begin{align*}
r = \left(
  m \,
  \left\lfloor
  \frac{1}{\lceil \log_2(n + 1) \rceil + 1}
  \right\rfloor
  - 1
\right).
\end{align*}
Note that this resolution $r$ progressively decreases with record depth $n$.

In describing the CRPR algorithm, we will build off the properties of the RPR and GSNR algorithms established in sections \ref{sec:recency-proportional-resolution-algo} and \ref{sec:geom-seq-nth-root-algo}.
Under the CRPR, at any given point in time either the RPR or GSNR is currently active.
If RPR is active, resolution parameterization depends on record depth $n$.
Whichever algorithm is currently active enumerates retained observation time points.
Time points to delete can be calculated through set subtraction of of subsequential curated collection enumerations.
Because curated collection size is bounded, this procedure is $\mathcal{O}(1)$.
Asymptotic properties result solely from GSNR, as it constitutes the final destination of the CRPR stitched policy sequence.
Except when switching CRPR's active policy algorithm, we can also carry forward self-consistency assurances from the existing RPR and GSNR policy algorithms.
However, when switching CRPR's active policy algorithm, we do need to assess self-consistency.
Transitioned-to time point collections must be a subset of transitioned-from time point collections.
% As Theorem \ref{thm:curbed-recency-proportional-resolution-algo-self-consistency} recounts, self-consistency largely arises from peculiarities of stacking monotonically decreasing binary powers.
Self-consistency turns out to largely arise from peculiarities of stacking monotonically decreasing binary powers.


In application, the CRPR policy algorithm should be preferable to GSNR and RPR for nearly all scenarios that call for recency-proportional resolution under capped-size storage limitations.
Except when switching active policy, update implementation can be optimized by replacing the set subtraction procedure with the active policy algorithm's implementation.
It turns out such transitions exclusively occur at perfect power-of-two time points.

% \input{thm/curbed-recency-proportional-resolution-algo-self-consistency.tex}


==> text/body/annotation-algorithms/depth-proportional-resolution-algo.tex <==
\subsection{Depth-Proportional Resolution (DPR) Policy Algorithm}
\label{sec:depth-proportional-resolution-algo}

The depth-proportional resolution policy algorithm affiliates even coverage over record history and capped extant record size.
To accomplish this, depth-proportional resolution approximates the cadenced spacing of retained observations at a gap width proportional to record depth.
An equivalent interpretation of DPR strategy would be interspersal of the historical record with a fixed number of waypoints.

Because observation time points are immutable after the fact, translating this naive DPR plan to a rolling, ``online'' basis necessitates a further consideration.
To conservatively maintain resolution guarantees, it is acceptable to error on the side of caution by choosing gap sizes smaller than naively supposed.
This allows a simple trick for policy self-consistency: flooring gap sizes to the next lower power of two.
Note that, under this scheme, when gap size slackens it will double.
Note also that multiples of a binary power subsume multiples of higher binary power.
So observations at slackened-to intervals always remain, having been retained as way points under the phased out gap size.
As intuition, therefore, the full DPR policy algorithm can be conceived of through a simple principle: successive eliminations of every other retained observation when a capacity threshold is reached.

Binary floor approximation exhibits another useful property: policy algorithm property distortions can be bounded by a constant.
With respect to the initial naive supposition, gap width is at most halved.
So, extant record count is at most doubled.
We structure parameterization of the DPR policy algorithm to account for divagation from binary flooring.
Policy algorithm behavior proceeds from a specified minimum gap count among retained observations, $r$.
(Note that $r$ also corresponds to minimum the number of distinguishable granules over record history.)
An absolute resolution guarantee of at least $n/r$, with $n$ as record depth, follows.
Further resulting is a constant extant record size order of growth, capped as extant observation count capped at $2r$.

Algorithm \ref{alg:depth-proportional-resolution-algo-enum-retained-ranks} provides enumeration of retained time points under the DPR scheme.
Although enactment can be parsimoniously formulated as set subtraction between enumerations at successive time points with $\mathcal{O}(1)$ complexity, Algorithm \ref{alg:depth-proportional-resolution-algo-gen-drop-ranks} addends a more expedient approach.
% Theorems \ref{thm:depth-proportional-resolution-algo-uncertainty-bound} and \ref{thm:depth-proportional-resolution-algo-space-complexity} cover extant record size order of growth and resolution guarantorship, respectively.
Figure \ref{fig:retention-policies} includes a time-lapse of the extant record under the DPR policy algorithm.

To streamline exposition, we have presented a bare-bones approach to provision of depth-proportional resolution where the entire record is simultaneously decimated by a factor of two upon reaching capacity.
This procedure results in regular episodes where extant record instantaneously halves.
Likely, such fluctuation would be undesirable in most use cases.
Many prescriptions for constant space complexity will arise from fixed memory allocation.
Such reserved memory cannot typically be use for other purposes, so maximization of space usage minimizes waste.
Occupying only half of bounded capacity clearly comes out on the ``use it or lose it'' downside.

An alternate ``tapered'' variant of the depth-proportional resolution algorithm can be easily defined to remedy this space-usage quirk.
Instead of all at once, the tapered approach eliminates phased-out observations one by one as new observations accrue.
% Supplementary Section \ref{sec:depth-proportional-resolution-tapered-algo} details this tapered DPR policy algorithm.
% TODO: ADD SECTION ^^^
The accompanying \texttt{hstrat} software library implements both variants.

% \input{alg/depth-proportional-resolution-algo-pred-keep-rank.tex}.
\input{alg/depth-proportional-resolution-algo-enum-retained-ranks.tex}
\input{alg/depth-proportional-resolution-algo-gen-drop-ranks.tex}
% \input{thm/depth-proportional-resolution-algo-space-complexity.tex}
% \input{thm/depth-proportional-resolution-algo-uncertainty-bound.tex}


==> text/body/annotation-algorithms/fixed-resolution-algo.tex <==
\subsection{Fixed Resolution (FR) Policy Algorithm}
\label{sec:fixed-resolution-algo}

The fixed resolution (FR) policy algorithm adopts a simplistic strategy: retain observation time points at intervals of a user-specified factor $r$.
This procedure equates to naive downsampling via decimation \citep[p. 31]{crochiere1983multirate}.
We include discussion of this policy algorithm primarliy for completeness.

The procedures to decide eliminated time points during the update process and to enumerate retained observation times are trivial.
Pruning targets time points that are not multiples of the fixed resolution $r$ and enumeration traverses time points at an even stride $r$ until reaching record depth.
% Algorithms \ref{alg:fixed-resolution-algo-gen-drop-ranks} and \ref{alg:fixed-resolution-algo-enum-retained-ranks} provide these procedures formally.

Unsurprisingly, extant record size order of growth is $\mathcal{O}(n)$.
A simple justification can be given: record depth $n$ provides an upper bound for extant record size because, being strictly subtractive, pruned size cannot exceed record depth.
Likewise, the downsampling factor $r$ enforces an upper bound $r$ on gap size between retained observations.
Any larger gap size would require at least one time point multiple of $r$ to have been discarded.
% \input{thm/fixed-resolution-algo-space-complexity.tex}
% \input{thm/fixed-resolution-algo-uncertainty-bound.tex}

The FR policy algorithm provides stable absolute accuracy indefinitely.
Such an approach will be necessary for scenarios that can tolerate only certain observational uncertainties.
However, because extant record size grows linearly this policy would not suit applications expecting long observational duration, high-frequency observation, or storage limitation.
Figure \ref{fig:retention-policies} includes a time-lapse of the extant record under the FR policy algorithm.

% TODO fill in if time available
% \input{alg/fixed-resolution-algo-gen-drop-ranks.tex}
% \input{alg/fixed-resolution-algo-enum-retained-ranks.tex}


==> text/body/annotation-algorithms/geom-seq-nth-root-algo.tex <==
\subsection{Geometric Sequence $n$th Root (GSNR) Policy Algorithm}
\label{sec:geom-seq-nth-root-algo}

% The geometric sequence $n$th root (GSNR) policy algorithm tackles recency-proportional uncertainty objectives within a fixed memory capacity constraint.  is that ok??????? yeah that looks good!! fixed-size memory? among observations? i like it!
The geometric sequence $n$th root (GSNR) policy algorithm arranges recency-proportional gap sizes among a capped-size set of retained observations.
% Although recency-proportional gap size will not be bounded below a fixed threshold in this context, GSNR seeks to minimize it to the extent possible.
Although recency-proportional gap size will not be bounded below a fixed threshold in this context, GSNR seeks to minimize gap size as much as possible.

Recall that the recency-proportional policy algorithm (RPR) exhibits logarithmic growth in extant record size with respect to record depth $n$.
When an increased order of magnitude depth is reached, additional observations must be retained under the RPR algorithm.
For $a = \log_b(n)$, $a$ is proportional to extant record size.
Equivalently, $b^a = n$.
Under RPR, growth in extant record size can be roughly conceptualized as related to insufficiency of the base $b$ to reach $n$ within $a$ multiplicative steps.
Growth in $a$ --- i.e., additional multiplication by $b$ --- can be thought of in terms of adding a level of structural hierarchy within the layout of retained observations.
As $n$ increases, additional levels of structural hierarchy become necessary.
These additional hierarchical levels increase extant record size.
% Put another way, progression of the policy algorithm accommodates additional appending an additional level of hierarchy.
% ELD: I feel like I was supposed to come away from this paragraph understanding what problem GSNR is trying to solve, but I don't

In order to prevent such unbounded growth, the GSNR policy algorithm fixes the number of hierarchical levels $a$ and accommodates additional record depth by adjusting the multiplicative factor $b$.
This scheme can be imagined enforcing as arrangement of $a$ exponentially-spaced target points along the historical record.
% ELD: I know we don't have time or space, but I think a little picture of this would help a lot
As time elapses, the quantity of target points remains constant.
The target points shift to fill $n$ by increasing their exponential spacing factor $b$.
The necessary magnitude of $b$ works out as $b = n^{1/a}$.
Target ages therefore correspond to $n^{0/a}, n^{1/a}, \ldots, n^{a/a}$.
This geometrically-spaced target point sequence eponymizes the GSNR policy algorithm.
Converting observation age to absolute time point, targets span $n - n^{0/a}, n - n^{1/a}, \ldots, n - n^{a/a}$.

% ELD: It might be worth trying to sign-post earlier that this algorithm is the way it is because that happens to work well, and that its not something that should be obvious to the audience

Now, attention turns to exploiting the $n$th root geometric targets to define a retention policy.
We will break the problem down to consideration of one individual target point $n - n^{x/a}$.
Under the constraint of $\mathcal{O}(1)$ total space for curated observations, we can only curate a fixed number of observations per target point.
We will seek to curate a fixed size collection of retained observations to bound gap size past the target point below $n^{x/a}$.

By nature of definition, target point times advance monotonically.
As a consequence, a retained observation can remain behind a target point indefinitely.
We will incorporate such coverage into our design --- let's call such a point behind the target the ``backstop'' $\beta$.
% Because the target point shifts with record depth, but retained time points are immutable, no retained backstop time point can exactly track the target point.
% ELD: Maybe "use" instead of "reach for"? Also maybe power of 2 instead of binary power? It took me a while to parse what a binary power is
% Instead, we will follow the vein of the RPR policy algorithm and the depth-proportional resolution policy algorithm and reach for a binary power.

We will use a power of 2 trick to maintain backstop coverage.
To begin, let us take the binary floor of half $n^{x/a}$,
% ELD: I'd either make this sentence have more intuition or cut it.
% TODO we should probably define binary floor in preliminaries and refer there
% addendum: we no longer have preliminaries
\begin{align*}
  \kappa(n)
  &=
  2^{\lfloor \log_{2}(n^{x/a}/2) \rfloor}.
\end{align*}
We will retain recent time points that are multiples of this value $\kappa$.
Note that $n$ strictly increasing implies $\kappa(n)$ monotonically increasing.

Let's define a floor $B$ to help place our backstop $\beta$,
\begin{align*}
  B(n)
  &=
  \max \left(
    n - \left\lceil  \frac{3n^{x/a}}{2} \right\rceil,
    0
  \right)
\end{align*}
By design, $B$ precedes target point $n - n^{x/a}$.
Again, with $x < a$, $n$ strictly increasing implies $B(n)$ monotonically increasing.

Rounding $B$ up to the next time point aligned to cadence $\kappa$ gives our backstop time point $\beta$,
\begin{align*}
  \beta(n)
  &=
  B(n) + \big(-B(n) \bmod \kappa(n)\big).
\end{align*}
% ELD: there's a weird gap in this equation, but it's probably not worth worrying about
% MAM: latex mod formatting is always weird and ugly
% SRP: \bmod is quirky and cute :3
It can be shown that $\beta(n) \leq n^{x/a}$.
Because $B(n)$ is monotonically increasing, $\beta(n)$ is as well.

We will retain the time point set $S_x$ comprising multiples of $\kappa$ at or after the backstop $\beta$,
\begin{align*}
  S_x(n) = \{\, t \mid \beta(n) \leq t < n \text{ and } t \mod \kappa(n) = 0 \,\}.
\end{align*}

Why are time points $S_x(n)$ guaranteed to be a subset of $S_x(n-1) \cup \{n\}$ (i.e., self consistency)?
Consider several non-mutually exclusive possible scenarios that could occur when transitioning from $n - 1$ to $n$,
\begin{enumerate}
  \item $\kappa$ changes: $\kappa(n - 1) \neq \kappa(n)$.

  Because $\kappa$ is monotonically increasing, $\kappa(n - 1) < \kappa(n)$.
  Binary flooring procedures have ensured $\kappa(n - 1)$ and $\kappa(n)$ are perfect powers of 2.
  Thus, $\kappa(n)$ is an even multiple of $\kappa(n - 1)$.
  So,
  \begin{align*}
    &\{\, t \mid \beta(n) \leq t < n \text{ and } t \mod \kappa(n) = 0 \,\}\\
    &\subseteq \{\, t \mid \beta(n) \leq t < n \text{ and } t \mod \kappa(n - 1) = 0 \,\}.
  \end{align*}
  Also, because $\beta$ monotonically increasing, $\beta{n - 1} \leq \beta{n}$.
  
  In conjunction, these stipulations give us $S_x(n) \subseteq \{S_x(n - 1), n\}$.
  % ELD: indentation is kind of wonky here

  \item $\beta$ changes: $\beta(n - 1) \neq \beta(n)$.

  Because $\beta$ is monotonically increasing, $\beta(n - 1) < \beta(n)$.
  We have $\beta(n) \mod \kappa(n) = 0$.
  Because $\kappa(n)$ is an even multiple of $\kappa(n - 1)$, we have $\beta(n) \mod \kappa(n - 1) = 0$.
  This implies $\beta(n) \in S_x(n - 1)$.
  Because $\beta$ monotonically increasing, change in $\beta$ strictly shrinks $S_x(n)$.

  \item $n \mod \kappa(n) = 0$

  Then the observation at time point $n$ is claimed for inclusion within $S_x(n)$.
  It is available, having just presently occurred.

\end{enumerate}

Note that if none of the above occur, then $S_x(n - 1) = S_x(n)$.
Any combination of the above maintains $S_x(n - 1) \in \{S_x(n), n\}$
% Theorem \ref{thm:geom-seq-nth-root-algo-self-consistency} details this point.


Why does this construction for target $n^{x/a}$ satisfy our $\mathcal{O}(1)$ space complexity constraint?
It can be shown that $|S_x(n)| \leq 6$.
This stems from cadence $\kappa$ as the binary floor of half $n^{x/a}$ (at most a quartering reduction) and backstop $\beta$ set at most $3/2 \times n^{x/a}$ time points back.

% Because cadence $\kappa$ is the binary floor of half $n^{x/a}$, we have $n^{x/a} \leq 4\kappa$.
% Recall that $\beta \geq n - 3 n^{x/a} / 2$.
% Remark that
% \begin{align*}
% |S_x(n)|
% = \lfloor \frac{n - \beta}{\kappa} \rfloor.
% \end{align*}

% Relaxing the integer floor,
% \begin{align*}
% |S_x(n)|
% \leq \frac{n - \beta}{\kappa}.
% \end{align*}

% Substituting inequalities,
% \begin{align*}
% |S_x(n)|
% &\leq 4\frac{n - \beta}{4\kappa}\\
% &\leq 4\frac{n - \beta}{n^{x/a}}
% \end{align*}

% and then

% \begin{align*}
% |S_x(n)|
% \leq 4\frac{n - \Big(n - 3 n^{x/a} / 2\Big)}{n^{x/a}} \\
% \leq 4\frac{3 n^{x/a} / 2}{n^{x/a}} \\
% \leq 4 \times \frac{3}{2} \\
% \leq 6.
% \end{align*}
% Theorem \ref{thm:geom-seq-nth-root-algo-space-complexity} details this point.

Why does this curated set for target $n - n^{x/a}$ satisfy our gap size bound $n^{x/a}$?
Because cadence $\kappa \leq \frac{n^{x/a}}{2}$, gap size satisfies the bound.
Because backstop $\beta \leq n - n ^{x/a}$, the target time point is covered within the cadenced range.
% Theorem \ref{thm:geom-seq-nth-root-algo-uncertainty-bound} details this point.

We bring curated sets for each target point together in a set union to produce the overall GSNR retained set $R$,
\begin{align*}
  R(n)
  &=
  \bigcup_{i=0}^{a} S_i(n).
\end{align*}
Note that under this construction, policy algorithm self-consistency and extant record size bounds follow from those shown for constructions for individual targets $n^{x/a}$.
\footnote{
A strict upper bound of $6a + 2$ for extant record size can be calculated, although we do not demonstrate it here.
}
Time points that should be dropped to enact the GSNR policy algorithm follow from set subtraction between $R(n)$ and $R(n+1)$.

We have discussed resolution guarantees for individual target point constructions, but what resolution guarantee is afforded overall for an arbitrary time point $t$ with age $g = n - t$?
For such a time point $t$, the tightest resolution guarantee is that of the next older target point.
Taking
\begin{align*}
\alpha = n^{1/a}
\end{align*}
the age of the next older target time point will be
\begin{align*}
\alpha^{ \lceil \log_{\alpha} g \rceil },
\end{align*}

By the target time point resolution guarantee we established earlier, the gap size provided at this target time point is bounded by its age.

Observe that, at most, the next older target time point age will be a factor of $\alpha = n^{1/a}$ greater than $g$.
So, the worst case absolute provided gap size is
\begin{align*}
\alpha \times g = n^{1/a} \times g.
\end{align*}

Worst case recency-proportional gap size is therefore $n^{1/a}$.

Figure \ref{fig:retention-policies} includes a time-lapse of the extant record under the GSNR policy algorithm.
The distinguishing feature of the GSNR policy algorithm is its sustained effort to minimize recency-proportional gap size without unbounded record size growth.
% ELD: What does indefinitely mean here?
This lends it to very-long duration applications.
% However, before very-deep record depths, we have observed that recency-proportional resolution tends to better distribute equivalent numbers of retained observations.

% \input{thm/geom-seq-nth-root-algo-self-consistency.tex}
% \input{thm/geom-seq-nth-root-algo-space-complexity.tex}
% \input{thm/geom-seq-nth-root-algo-uncertainty-bound.tex}

% \input{alg/geom-seq-nth-root-algo-gen-drop-ranks.tex}
% \input{alg/geom-seq-nth-root-algo-pred-keep-rank.tex}
\input{alg/geom-seq-nth-root-algo-enum-retained-ranks.tex}


==> text/body/annotation-algorithms/recency-proportional-resolution-algo.tex <==
\subsection{Recency-proportional Resolution (RPR) Policy Algorithm}
\label{sec:recency-proportional-resolution-algo}

This streaming curation algorithm's properties fall between the properties of the fixed resolution (FR) and depth-proportional resolution (DPR) policy algorithms, covered in the immediately preceding sections.

Recall that the DPR policy algorithm's gap widths grow in linear proportion to record depth.
In contrast, the fixed resolution algorithm's gap width remains constant below a specified bound across record depths.

The recency-proportional resolution (RPR) policy algorithm bounds gap width to a linear factor of layer age (i.e., time steps back from the newest layer).
Suppose $n$ observations have elapsed.
% set k as age and explain that then replace n - m
% annotate-equations (latex math annotation?)
Then, for a user-specified constant $r$, no gap width for layer $m$ will exceed size
\begin{align}
  \left\lfloor \frac{n - m}{r} \right\rfloor.
  \label{eqn:rpr-gap}
\end{align}
Resolution at each layer widens linearly with record depth.
Consequently, resolution widens in linear proportion to layer age.
Resolution for any given layer age, however, remains constant for all record depths.

The FR and DPR policy algorithms exhibit $O(r)$ and $O(rn)$ extant record orders of growth, respectively.
We will show extant record order of growth as $O(r\log{n})$ under the recency-proportional resolution policy algorithm.

Algorithm \ref{alg:recency-proportional-algo-gen-drop-ranks} enumerates time points of dropped observations under the RPR policy algorithm.
Figure \ref{fig:retention-policies} includes a time-lapse of the extant record under this policy algorithm.

The extant record is determined iteratively, beginning at observation time zero --- which is always retained.
Per Equation \ref{eqn:rpr-gap}, gap width to the next retained observation can be at most $\lfloor n/r \rfloor$ sites, where $n$ is record depth.
Although selecting to retain the $\lfloor n/r \rfloor$ observation time observation would satisfy policy resolution guarantees, a slight complication is necessary to ensure that retained observations have previously been deleted.
A fuller self-consistency rationale will follow, but in short gap width is floored to the next lower power of two,
\begin{align*}
  2^{\lfloor \log_{2}\left(\frac{n}{r}\right) \rfloor}.
\end{align*}
The next iteration repeats the procedure from the newly retained observation time instead of observation time zero.
Iteration continues until reaching the newest observation.

The set of observations to eliminate can be calculated from set subtraction between enumerations of the historical record at time points $t-1$ and $t$.
So, update time complexity follows from extant record enumeration time complexity, which turns out to be $O(\log n)$.
We provide a tested, but unproven, constant-time pruning enumeration implementation in the \texttt{hstrat} library, but will not cover it here. % mention why?
The extant record order of growth $O(\log n)$ also follows closely from the record enumeration algorithm, as detailed in Theorem \ref{thm:recency-proportional-resolution-algo-space-complexity}.

% TODO figure?

Why does flooring step sizes to a binary power ensure self-consistency?
Let us begin by noting properties applicable to all layers $l$,
\begin{enumerate}
\item gap width provided at retained layer $l$ increases monotonically as record depth grows,
\item the retained observation preceding or at $l$ has observation time at an even multiple of surrounding gap widths, and
\item all observations at time points that are multiples of gap width past $l$ up to the newest observation are retained.
\end{enumerate}
Observe that gap width decreases monotonically with decreasing layer age (i.e., increasing layer recency).

Properties 2 and 3 occur as a result of stacking monotonically-decreasing powers of two.
Subsequent smaller powers of two tile evenly to all multiples of a larger power of 2, giving property 3.
Conversely, preceding larger powers of 2 can be evenly divided by succeeding smaller powers of 2, ensuring that the edges of smaller powers of 2 gaps occur at even multiples of their gap width, giving property 2.

Under the binary flooring procedure, when gap size increases at a layer it will double (or quadruple, octuple, etc.).
Availability of the new gap endpoint after a gap size increase is guaranteed from the tiling properties due to that endpoint being an even multiple of original step size.
% Theorem \ref{thm:recency-proportional-resolution-algo-self-consistency} uses inductive proof-by-contradiction to show this self-consistency.

The RPR policy algorithm provides stable relative accuracy indefinitely.
This makes it particularly attractive in phylogenetic tracking scenarios using hereditary stratigraphy where guarantees about branch length accuracy are critical.
At comparable annotation sizes, we have found that recency-proportional distribution of gap widths outperforms even gap width distribution in phylogenetic information recovery \citep{moreno2022hereditary}.
Preliminarily, maintaining 3\% relative precision appears sufficient to eliminate most bias from reconstruction error on phylogenetic metrics \citep{moreno2023toward}.
%TODO add details about coalescent theory being a good idea for recency-proportional

The RPR policy algorithm's indefinite stability may be particularly useful in scenarios of indefinite or indeterminate record keeping duration.
Although annotation extant record size grows unboundedly, logarithmic memory usage growth is manageable in most practical scenarios.
However, this policy would not suit applications with hard caps on annotation size (e.g., fixed memory footprint digital genomes).

\input{alg/recency-proportional-resolution-algo-gen-drop-ranks.tex}
% \input{alg/recency-proportional-resolution-algo-pred-keep-rank.tex}
% \input{alg/recency-proportional-resolution-algo-enum-retained-ranks.tex}

% \input{thm/recency-proportional-resolution-algo-self-consistency.tex}
\input{thm/recency-proportional-resolution-algo-space-complexity.tex}
% \input{thm/recency-proportional-resolution-algo-uncertainty-bound.tex}


==> text/body/experimental-evaluation.tex <==
\section{Experimental Evaluation} \label{sec:experimental-evaluation}

TODO: add content from alife paper here


==> text/body/introduction-scraps.tex <==
Digital evolution is a field of research that sits at the intersection of evolutionary biology and machine learning.
By instantiating evolution in computers, researchers are able to advance our knowledge of both subjects.
Increasing computational power is essential to many advances in digital evolution and, more broadly, artificial life \citep{ackley2014indefinitely}.
In fact, a central motif in the field --- the problem of open-ended evolution, which asks how and if closed systems can indefinitely yield new complexity, novelty, and adaptation --- is inexorably intertwined with computational scale, and has been implicated as meaningfully compute-constrained in at least some systems \citep{taylor2016open,channon2019maximum}.
It is not an unreasonable possibility that orders-of-magnitude changes in computational power could induce qualitative changes in digital evolution and artificial life systems \citep{moreno2022engineering}, analogously to the renaissance of deep learning with the advent of GPGPU computing \citep{krizhevsky2012imagenet}.

However, contemporary advances in computer hardware have been a double-edged sword.
Fundamental physical limitations have essentially curtailed transformative progress in individual processing elements \citep{sutter2005free}.
Instead, the frontier of raw compute power in high-performance computing (HPC) has largely been advanced by increasing processing core counts \citep{morgenstern2021unparalleled}.
Leveraging parallel and distributed computing power for digital evolution will require continuing work adapting existing methodologies oriented towards serial processing to suit these hardware trends.

% On the flip side, economization and miniaturization has driven broad dissemination of computing capability through the Internet of Things (IoT) revolution \citep{rfc7228,ojo2018review}.
% A notable pattern cuts across some facets of both fringes: absolute reduction or tightening or relative tightening in resources and capabilities per processing element, particularly with respect to the capacity, latency, or bandwidth of memory and storage.
% Along the march to exascale HPC, processing capacity growth (e.g., FLOPS) has outpaced memory performance and capacity --- particularly with respect to hardware accelerators \citep{kogge2013exascale,khan2021analysis}.
% This ``memory wall'' bottlenecks throughput unless memory access volume is kept sufficiently low in proportion to processing workload (i.e., high ``arithmetic'' or ``operational'' intensity is achieved) \citep{obviousmemorywall,mckee2004reflections,ROOFLINEMODEL2008Berkley}.
% Analogous performance trajectories have played out with respect to data storage \citep{heldens2020landscape,kunkel2014exascale}, imposing an analogous ``storage wall'' bottleneck \citep{hu2016storage}.
% Recent introduction of the Cerebras Wafer-Scale Engine epitomizes the double-edged nature of recent HPC trends: this accelerator packages an astounding 850,000 computing elements onto a single piece of silicon, but restricts endows each with a modest 48kb of memory and provisions an exclusively-local mesh communication model \citep{cerebras2021wafer,lauterbach2021path}.

% The intersection of these observations is that despite relentless technological advancement, severely resource-limited computation will persist.
% In fact, in some domains technological progress has actually elevated the relevance of resource-limited computation.
% These trends, and the wider context of surging generation of digital data \citep{bhat2018data}, demand attention to algorithmic strategies to triage memory/storage-capacity gaps.

% ELD: Moving this to beginning
% Burgeoning computational power has been broadly envisaged as driving force in advancing the field of digital evolution and, more broadly, artificial life \citep{ackley2014indefinitely}.
% In fact, a central motif in the field --- the problem of open-ended evolution, how and if closed systems can yield indefinitely yield new complexity, novelty, and adaptation --- is inexorably intertwined with computational scale, and has been implicated as meaningfully compute-constrained in at least some systems \citep{taylor2016open,channon2019maximum}.
% It is not an unreasonable possibility that orders-of-magnitude changes in computational power could induce qualitative changes in digital evolution and artificial life systems \citep{moreno2022engineering}, analogously to the renaissance of deep learning with the advent of GPGPU computing \citep{krizhevsky2012imagenet}.
% To accomplish such, however, will require contending with scaling challenges induced by aforementioned hardware trends.

% ELD: TODO: consider cutting this paragraph
Parallel and distributed computing is, indeed, already widely leveraged in digital evolution.
Applications range from processing entirely independent evolutionary replicates across compute jobs \citep{dolson2017spatial, hornby2006automated}, to data-parallel fitness evaluation of single individuals over independent test cases using hardware accelerators \citep{harding2007fast_springer, langdon2019continuous}, to application of primary-subordinate/controller-responder parallelism to delegate costly fitness evaluations of single individuals \citep{cantu2001master,miikkulainen2019evolving}.
In recent years, Sentient Technologies spearheaded evolutionary computation projects on an unprecedented computational scale, comprising over a million heterogeneous CPUs from time-available providers capable of a peak performance of 9 petaflops \citep{miikkulainen2019evolving,gilbert2015artificial,blondeau2009distributed}.

Although highlighted as key to the future of the field, fully decentralized, highly-distributed approaches such as island models \citep{bennett1999building,schulte2010genetic} and mesh-computing approaches prioritizing dynamic interactions \citep{ray1995proposal,ackley2018digital,moreno2021conduit} have been less thoroughly developed.
A major barrier to effective applications of the fully-distributed paradigm is the difficulty of observing the state of the system. 
In the absence of a global population-level view, the course of evolution becomes much more challenging to study --- undercutting the objective of these systems as an experimental tool.
A prime example of this problem is the difficulty of recording phylogenies (i.e. ancestry trees) in distributed systems.

\subsection{Phylogeny recording}

Although phylogenetic analysis is a powerful tool for understanding digital evolution \citep{dolson2020interpreting}, typical approaches are particularly difficult to scale.
Most existing analyses use direct lineage tracking, where a centralized data structure collates individual reproduction events to produce a complete, perfect phylogenetic record \citep{dolson2023phylotrackpy}.
However, this approach requires centralized data storage, which performs poorly in distributed computing environments (see Sections \ref{sec:perfect-tracking-distrbuted} and \ref{sec:perfect-tracking-pruning-distrbuted} for more information).

The problem of recording phylogenies in a distributed context generalizes beyond digital evolution.
Phylogenies can be used to understand any process in which a population of objects exist and those objects are sometimes replicated (with or without modification).
Indeed, phylogenetic techniques have been used to study the routes through which digital image misinformation and computer viruses spread \citep{friggeri2014rumor,cohen1987computer}.
As in digital evolution, such studies generally rely on centralized tracking and are thus inhibited when it is not possible.

% As such, hereditary stratigraphic techniques certainly possess some potential afford experimenters visibility into the otherwise cloistered processes through which such digital artifacts spread.
% Notably, though, such experiments would predicate on some level of influence over the artifact copy process in to ensure dispatch of the hereditary stratigraphic update process and the absence of actors with motivation and capability to antagonistically deface annotation data.


%TODO we could probably add some citations/examples about why phylogenetic tracking is important
% AND how perfect phylogenetic tracking is super powerful at doing otherwise unimaginable analyses
% probably pilfer phylotrackpy JOSS paper for ideas
% TODO also tie in the algorithmic analysis of phylogenies here
% ELD: TODO: See if any of the points below aren't made in the perfect tracking section, and if not move them
% However, long distance, potentially many-hop, transmission of reproduction event records to a centralized data store introduces potentially significant amounts of communication overhead and bottlenecking.
% The necessity to propagate extinction notifications at runtime so that records of lineages without extant descendants can be pruned away to prevent runaway memory use imposes additional communication overhead.
% Further, at large enough scales, node failures become inevitablies rather than inconveniences and, at even larger scales, the cost of attempting full recovery from node dropout to prevent data loss could become high enough to conceivably preclude forward simulation progress \citep{cappello2014toward}.
% Within the perfect-tracking paradigm, individual missing relationships could potentially entirely disjoin knowledge of how large portions of phylogenetic history relate.
% This sensitivity to data loss poses a second major challenge in scaling perfect tracking.

% Looking to natural systems, however, fruitful efforts across generations of systematic biologists evidence the viability of robust phylogenetic analyses from data generated through fully-distributed processes.
Looking to natural systems, it is clear that robust phylogenetic analyses can be conducted on data generated through fully-distributed processes.
% An alternate approach to studying phylogenetic dynamics in distributed systems, therefore, can be entertained: post-hoc inference from heritable data rather than centralized tracking.
Inspired by systematic biology, we can consider post-hoc inference from heritable data as an alternative tocentralized tracking.
% Although such analyses can passably be accomplished solely from direct analysis of pre-existing, functional digital genome contents \citep{moreno2021case}, such algorithms do not generalize across diverse digital evolution systems and suffer from many of the complications that plague phylogenetic analyses of biological systems.
Although such analyses can be accomplished solely from pre-existing, functional digital genome contents \citep{moreno2021case}, such algorithms do not generalize across diverse digital evolution systems and suffer from many of the complications that plague phylogenetic analyses of biological systems.
An intriguing proposition arises: how might a genetic representation be designed to maximize ease and efficacy of phylogenetic reconstruction?

If sufficiently compact, such a representation could be attached as a non-functional annotation to facilitate phylogenetic inference over genomes of interest.
This line of reasoning led to the recent development of ``hereditary stratigraphy'' methodology, which associates digital genomes with heritable annotations specially designed to provide universal system-invariant phylogenetic reconstruction with well-defined, tunable expectations for inference accuracy
\citep{moreno2022hereditary}.

%TODO should this whole bit move to methods?
% ELD: Yeah I think so
% The principal aspects of hereditary stratigraphy can be sketched briefly.
% However, briefly sketching a more obvious alternate approach provides a point of reference more familiar to most readers' intuiition.
% A simple heritable annotation to enable relatedness estimation would be a fixed--length bitstring under neutral drift by bit flip mutation.
% As lineages diverge from a common ancestor, gradual mutational accumulation probabilistically causes the hamming distance between annotations to diverge.
% Therefore, hamming distance between these annotations can be used as inferential proxy: more mismatching sites imply less relatedness between two annotated digital organisms.
% Unfortunately, this model suffers from several serious drawbacks in application as a tool for relatedness estimation, including difficulty resolving uneven lineage branch lengths and difficulty parameterizing the model for effective inference over greatly varying generational scales.

% Hereditary stratigraphy annotations employ a systematic update process at generational turnovers instead of a stochastic mutational process as described above.
% Each generation, a new fixed-length packet of randomly-generated data is appended to inherited annotations.
% These stochastic ``fingerprints,'' typically sized on the order of a few bits or bytes, serve as a sort of checkpoint for lineage identity at a particular generation.
% At future time points, extant annotations will share identical fingerprints for the generations they experienced shared ancestry.
% Estimation of the last common ancestor generation is straightforward: the first mismatching fingerprints denote the end of common ancestry.
% However, note that overestimation of relatedness can occur due to spurious fingerprint collision events (i.e., where strata happen to share the same randomly-generated value by chance); the probability of such events depends on ``fingerprint'' width.
% The nomenclature of ``hereditary stratigraphy'' was chosen through analogy to geological layering processes.

\subsection{Hereditary stratigraphy}

The crux of hereditary stratigraphy is that each at generation, a new fixed-length packet of randomly-generated data is appended to inherited annotations.
These stochastic ``fingerprints,'' typically sized on the order of a few bits or bytes, serve as a sort of checkpoint for lineage identity at a particular generation.
At future time points, extant annotations will share identical fingerprints for the generations they experienced shared ancestry.

Interestingly, a similar technique was used by \cite{libennowell2008tracing} to trace global dissemination of chain emails.
These researchers applied \textit{post-hoc} methods to reconstruct estimated phylogenies of the propagation of two chain mail messages.
These phylogenies then served as a reference to tune agent-based models, ultimately yielding a remarkable elucidation of email user behavior and underlying social dynamics.
Interestingly, this study's reconstructions were solely enabled by a special peculiarity of the two sampled messages: they were email petitions.
Thus, users would append their name to the list before forwarding it on --- a mechanism strikingly similar to the broad strokes of hereditary stratigraphy.

Naive application of hereditary stratigraphy would produce indefinitely lengthening genome annotation size in direct proportion to generations elapsed.
To overcome this obstacle, hereditary stratigraphy prescribes a ``pruning'' process to discard strata on the fly as new strata are deposited.
Pruning reduces annotation size, but at the expense of introducing inferential uncertainty: the last generation of common ancestry between two lineages can be resolved no finer than the time points associated with retained strata.
Deciding which strata to discard is the main point of algorithmic interest associated with the technique.
In fact, this scenario turns out to be an instance of a more general class of online algorithmic problems we hereby term as ``streaming curation.''
In the context of hereditary stratigraphy, we refer to the decision-making rules that decide which retained strata to discard per generation as a ``stratum retention'' algorithm.
% ELD: TODO: is this correct or do we call them curation policy algorithms now?

% Putting ``hereditary stratigraphy'' techniques into practice requires a point of further consideration.
% Naive application of the approach described above would entail indefinitely lengthening genome annotation size in direct proportion to generations elapsed due to the creation of new ``fingerprint'' data each generation.
% To overcome this obstacle, hereditary stratigraphy prescribes a ``pruning'' process to discard strata on the fly as new strata are deposited.
% Note that pruning reduces annotation size, but at the expense of introducing inferential uncertainty: the last generation of common ancestry between two lineages can be resolved no finer than the time points associated with retained strata.
% Deciding which strata to discard when proves to be the main point of algorithmic interest associated with the technique.
% In fact, as will be delved into a little further on, we find this scenario to be an instance of a more general class of online algorithmic problems we term as ``streaming curation.''
% In the context of hereditary stratigraphy, we refer to the decision-making rules that decide which retained strata to discard per generation as a ``stratum retention'' algorithm.


\subsection{Stratum retention}

The obvious core issue of stratum retention is how many strata to discard.
In many applied cases, it is desirable to keep the count of retained strata at or below a size cap indefinitely as generations elapse.
However, in some cases discussed later on, it may be desirable to allow a logarithmic growth rate of annotation size to guarantee upper bounds on inferential uncertainty.

Determining stratum retention strategy also raises a more subtle second consideration: what skew, if any, to induce on the composition of retained strata.
Strata from evenly-spaced time points may be retained in order to provide uniform inferential detail over the entire range of elapsed time points.
However, coalescent theory predicts that evolution-like processes will tend to produce phylogenies with many recent branches and progressively fewer more ancient branches \citep{nordborgCoalescentTheory2019, berestyckiRecentProgressCoalescent2009}.
Thus, fine inferential detail over more recent time points is usually more informative to phylogenetic reconstruction than fine detail over more ancient time points.
Thus, among a fixed-size retained sampling of time points, skewing the composition of retained strata to over-represent more recent time points would likely provide better bang for the buck with respect to reconstructive power.
Indeed, experiments reconstructing known lineages have shown that recency-skewing retention provides better quality reconstructions \citep{moreno2022hereditary}.
So, in addition to evenly-spaced retention, we consider retention allocations that yield gap widths between successive retained strata (and corresponding estimation uncertainty) scaled proportionately to those strata's depth back in history.

Because no single retention policy can meet requirements of all use cases, we present in Section \ref{sec:annotation-algorithms} a suite of complementary stratum retention algorithms covering possible combinations of retained stratum count order of growth and chronological skew.
We describe retention algorithms in terms of upper bounds on memory usage and inference uncertainty.

With respect to memory usage, we refer to guaranteed upper bounds as ``size order of growth'' in the asymptotic case with respect to elapsed generations or ``size cap'' in the absolute case.
We refer to bounds on spacing between retained strata a ``resolution guarantee.''
Resolution guarantee specification incorporates both the total number of generations elapsed and the historical depth of a particular time point in the stratigraphic record --- so, bounding is tailored within these particular circumstances.

%ELD: TODO: This said "three nutes and bolts consdierations" but there were only two. I changed it to say two, but is there one missing?
In addition to their particular size bounds and resolution guarantees, we demonstrate all proposed stratum retention algorithms satisfy two nuts and bolts algorithmic considerations:
\begin{enumerate}
\item \textbf{Tractability of directly enumerating deposition time of retained strata at any arbitrary generation.} Efficient computation of the deposition times retained at each time point provides a tractable reverse mapping from column array index to deposition generation.
  Such a mapping enables deposition generation to be omitted from stored strata, potentially yielding several-fold space savings (depending on the differentia bit width used).

\item \textbf{Stratum discard sequencing for ``self-consistency.''} 
  When you discard a stratum now, it won't be available later.
  If you need a stratum at a particular time point, you must be able to guarantee it hasn't already been discarded at any prior time point.

\end{enumerate}

% As a final spelling out of a critical conceptual point in discussion of stratum retention policies, note that size bounds and resolution guarantees are enforced across across all generations.
% This means stratum retention policies must manage ``online'' column composition across rolling generations.
% Indeed, for many use cases, resolution and column size guarantees will need to hold at all generations because the number of generations elapsed at the end of an experiment is often not known \textit{a priori} and the option of continuing a fixed-length experiment with evolved genomes is desired.
% This factor introduces a design subtlety: as generations elapse, deposited strata recede to increasingly ancient historical depth with respect to the current generation.
% Resolution guarantees may change along the way back.
% In those cases, cohorts of retained strata must, in dwindling, gracefully morph through a constrained series of retention patterns.

Note that size bounds and resolution guarantees are enforced across across all generations.
Thus, stratum retention policies must manage ``online'' column composition across rolling generations.
Indeed, for many use cases, resolution and column size guarantees will need to hold at all generations because the number of generations elapsed at the end of an experiment is often not known \textit{a priori} and the option of continuing a fixed-length experiment with evolved genomes is desired.
This factor introduces a design subtlety: as generations elapse, deposited strata recede to increasingly ancient historical depth with respect to the current generation.
Resolution guarantees may change along the way back.
In those cases, cohorts of retained strata must, in dwindling, gracefully morph through a constrained series of retention patterns.

\subsection{The streaming curation problem}

Stepping back, the online filtering obligations faced by hereditary stratigraph annotations are not unlike those faced by unattended data logger devices.
Both manage incoming observation streams on a potentially indefinite or indeterminate basis and both operate under storage space limitations.
Further, both are presumedly tasked to operate under some stipulation for time coverage, whether simply rolling full retention of most recent data within available buffer space \citep{fincham1995use}, dismissal of incoming data after storage reaches capacity \citep{saunders1989portable,mahzan2017design}, best-effort even coverage of the elapsed period, or otherwise.
Even high-capacity devices may experience overflow conditions when confronted with high-frequency data streams \citep{luharuka2003design}.

Restated explicitly, these scenarios confront a question of how to satisfactorily maintain a temporally representative cross section of observations that stream in on a rolling basis.
We propose this problem as the ``stream curation problem.''
For the sake of generalizability, Section \ref{sec:annotation-algorithms} organizes presentation of stratum retention algorithms through the lens of the streaming curation problem.
There has been some work to extend the record capacity of data loggers through application-specific online compression algorithms \citep{hadiatna2016design}, but to our knowledge the streaming curation problem has not been treated directly from either a theoretical or empirical vantage.
As low-end hardware continues to march toward the downscale and ubiquity of ``smart dust'' \citep{warneke2001smart}, we expect this problem will become increasingly relevant.

% Indeed, low-end hardware continues to march toward the downscale and ubiquity of ``smart dust'' \citep{warneke2001smart}.
% The ``Michigan Micro Mote'' constitutes a notable waypoint \citep{lee2012modular}.
% These devices occupy only a cubic millimeter of volume, but provision a mere 3 kb of retentive memory.
% Introduced in 2012, applications have since been explored across imaging, motion detection, pressure measurement, and electrocardiography monitoring \citep{lee2015review}.
% Taking for instance another more recent high-profile project, computational capacity was recently tucked into wireless sensor network devices adopting the form factor of dandelion parachutes \citep{iyer2022wind}.
% The chipset for these devices provisions 2 kilobytes of volatile flash memory --- and a mere 128 bytes of retentive memory \citep{microchip2014atiny20}.
% Even more striking is the advent of an epidermal physiological sensor equipped with carbon nanotube-based flash memory of a scant 48 bytes \citep{xiang2022epidermal}.
% The ever abiding race to plumb the very lower limits of technical feasibility seems likely to keep bare-bones computing modalities front and center within this engineering domain far into the future.

% Recalling earlier discussion of hardware trends, the accelerating ubiquitization of IoT hardware and, in particular, continuing downscaling toward smart dust call stream curation scenarios directly into play.

Some of the same curation policy algorithms we propose for stratum retention could also be useful in these cases.
For example, organization of IoT devices into wireless sensor networks is expected, in a considerable fraction of cases, to structure irregular device uplink schedules, such as the ``mobile sink'' paradigm \citep{jain2022survey}.
% The so-called ``mobile sink'' paradigm has risen to some prominence due to advantages with respect to power management, security, and network load management \citep{jain2022survey}.
Under this model, network base station(s) physically traverse the coverage area and transact with nearby sensor nodes.
Reliance on the mobile sink's patrol schedule potentially introduces uncertainty in data transfer schedules.
% TODO: One sentence on why our curation policies would help with this
Streaming curation may be particularly relevant to data management in surveillance devices such as doorbell or body-worn cameras, which have experienced notable market growth \citep{calacci2022cop,lum2019research}.
Recency-proportional retention may suit some applications, where time intervals of interest may be flagged well after the fact, but tend to bias toward the recent past.
% This approach could also align with the objectives of some accident recording devices.
% TODO this sentence sucks: rephrase
Finally, streaming curation may even pertain to record management in large capacity centralized storage systems in some scenarios \citep{bhat2018data}.

% It should also be noted that beyond connections to streaming curation, hereditary stratigraphy itself bears upon applications outside digital evolution modeling.
% Computer viruses and digital media also proliferate through replication, often outside the scope of direct centralized observability.
% Furthermore, understanding the dynamics of these phenomena is of significant scientific and societal interest \citep{aslan2020comprehensive,dupuis2019spread,ling2021dissecting}.
% Indeed, some research has reported on the routes through which digital image misinformation and computer viruses spread \citep{friggeri2014rumor,cohen1987computer}.
% Such studies generally rely on centralized tracking, which is not possible in many circumstances.
% A notable exception is work by \cite{libennowell2008tracing} to trace global dissemination of chain emails.
% These researchers applied \textit{post-hoc} methods to reconstruct estimated phylogenies of the propagation of two chain mail messages.
% These phylogenies then served as a reference to tune agent-based models, ultimately yielding a remarkable means elucidation of email user behavior and underlying social dynamics.
% Interestingly, this study's reconstructions were solely enabled by a special peculiarity of the two sampled messages: they were email petitions.
% Thus, users would append their name to the list before forwarding it on --- a mechanism strikingly similar to the broad strokes of hereditary stratigraphy.

% As such, hereditary stratigraphic techniques certainly possess some potential afford experimenters visibility into the otherwise cloistered processes through which such digital artifacts spread.
% Notably, though, such experiments would predicate on some level of influence over the artifact copy process in to ensure dispatch of the hereditary stratigraphic update process and the absence of actors with motivation and capability to antagonistically deface annotation data.


\subsection{Hereditary Stratigraphy} \label{sec:hereditary-stratigraphy}

Digital systems excel at copying and distributing information \citep{miller2001taking}.
Provenance among digital artifacts produced through copy operations can be represented as a tree of parent-child relationships (in this case, original-copy relationships).
The structure of digital ancestry trees can answer important questions pertinent to cybersecurity, misinformation, and cultural anthropology \citep{aslan2020comprehensive,dupuis2019spread,ling2021dissecting}.
To explain how and why such ancestry analysis might be accomplished, we next contrast direct ancestry tracking with distributed ancestry tracking, outline hereditary stratigraphy methodology for distributed ancestry tracking, and review applications of distributed ancestry tracking.

\subsubsection{Direct Ancestry Tracking}

Most work on ancestry trees of digital artifacts relies on centralized lineage tracking \citep{friggeri2014rumor,cohen1987computer,dolson2023phylotrackpy}.%
\footnote{A notable exception, \cite{libennowell2008tracing} exploit a serendipitous mechanistic opportunity to reconstruct global dissemination of chain emails --- discussed further below.}
Direct approaches to tracking replicator provenance in digital systems operate on this graph structure directly, distilling it from the full set of parent-child relationships over the history of a population to produce an exact historical account.

Unfortunately, typical lineage tracking is difficult to scale.
At scale, practical limitations preclude comprehensive records of replication events, which accumulate linearly with elapsed generations.
So, extinct lineages must be pruned.
Detecting lineage extinctions requires either (1) collation of all replication and destruction events to a centralized data store or (2) peer-to-peer transmission of extinction notifications that unwind a lineage's (possibly many-hop) trajectory across host nodes.
Both options oblige runtime communication overhead.
To boot, the perfect-tracking paradigm is fragile to single missing relationships --- these can entirely disjoin knowledge of how large portions of phylogenetic history relate.
This fragility makes direct lineage tracking highly sensitive to data loss and dynamic network topology rearrangements, which are ubiquitous at scale \citep{cappello2014toward,ackley2011pursue}.

\subsubsection{Motivation for Decentralized Ancestry Tracking}

Under an alternate framing, biological phylogenetics almost certainly constitutes the single most extensive investigation of artifact provenance ever conducted.
Decades of phylogenetics researchers have waged a vast and sophisticated campaign to stitch together millions of lines of descent via analysis of fossil records, phenotypic traits, and --- especially --- genetic information \citep{hinchliff2015synthesis,lee2015morphological}.
The successes of biological phylogenetics resoundingly demonstrate the viability of robust phylogenetic analyses over large, long-running, and fully-distributed systems.

Inspired by systematic biology, we can consider post hoc inference from heritable data as an alternative to direct tracking.
At core, biological processes of mutation, recombination, conjugation, transformation, transduction, and gene transfer induce patterns of heritable variation that can be mined to reveal historical relationships \citep{davis1992populations}.

Indeed, in digital systems with imperfect copy processes (e.g., digital evolution), phylogenetic reconstructions can be accomplished ad hoc, i.e., directly from copy artifacts themselves \citep{moreno2021case}.
However, this approach has major drawbacks ---
(1) ad hoc reconstruction algorithms are highly dependent on representational specifics so do not readily generalize;
(2) ad hoc approaches suffer from many of the complications that plague phylogenetic analyses of biological systems such as back mutation and mutational saturation;
(3) systems without mutational dynamics (i.e., perfect copies) entirely lack information on heredity.

The challenges associated with ad hoc ancestry estimation begs the question of how to design genetic material to optimize phylogenetic reconstruction.
If sufficiently compact, such a representation could be annotated onto artifacts of interest in order to facilitate phylogenetic inference.
This scheme assigns each artifact an annotation, with parents' annotations passed down to offspring artifact copies.

The recently developed ``hereditary stratigraphy'' methodology implements this approach, providing a design for heritable annotations that facilitate universal system-invariant phylogenetic reconstruction with well-defined, tunable expectations for inference accuracy \citep{moreno2022hereditary}.

\subsubsection{Mechanisms for Decentralized Ancestry Tracking}

The core mechanism of hereditary stratigraphy is accretion, and subsequent inheritance, of a new randomized data packet each copy generation.
These stochastic fingerprints, which we call ``differentia,'' serve as a sort of checkpoint for lineage identity at a particular generation.
At future time points, extant annotations will share identical differentia for the generations they experienced shared ancestry.
So, the first mismatched fingerprint between two annotations bounds their common ancestry.

To circumvent annotation size bloat, hereditary stratigraphy prescribes a ``pruning'' process to delete differentia on the fly as generations elapse.
This pruning, however, comes at a cost to inference power.
The last generation of common ancestry between two lineages can be resolved no finer than retained checkpoint times.
In the context of hereditary stratigraphy, we refer to the procedure for down sampling as a ``stratum retention algorithm'' and the resulting patterns of retained differentia as a ``stratum retention policy.''
Stratum retention algorithms must decide how many records to discard, but also how remaining records distribute over past time.
Discussion considers tuning stratum retention trade-offs elsewhere as an instance of the more general ``stream curation'' problem --- introduced separately below in Section \ref{sec:streaming-curation} and fully presented in Section \ref{sec:annotation-algorithms}:

Procedures for ancestry tree reconstruction from a population of stratigraph annotations follow from the same principle as pairwise annotation comparison, but merit some further elaboration.
Section \ref{sec:reconstruction-algorithm} provides a trie-based algorithm for this task.

\subsubsection{Distributed Ancestry Trees in Digital Evolution}

Digital evolution refers to computational systems that combine replication, mutation, and selection to instantiate an evolutionary process.
The field sits at the intersection of evolutionary biology, viz. simulation experiments, and machine learning, viz. heuristic optimization.
Within digital evolution, complications of distributed tracking have historically restricted most phylogenetic analyses to single-process or centralized leader/follower simulations.
Need for phylogenetic methods compatible with parallel and distributed simulation motivated original development of hereditary stratigraphy \citep{moreno2022hereditary}.

Computational scale matters in digital evolution and, more broadly, artificial life \citep{ackley2014indefinitely} --- particularly with respect to open-ended evolution (OEE), the question of how (and if) closed systems can indefinitely grow in complexity, novelty, and adaptation \citep{taylor2016open}.
OEE is inexorably intertwined with computational scale, and has been implicated as meaningfully compute-constrained in at least some systems \citep{channon2019maximum}.
It is not an unreasonable possibility that orders-of-magnitude changes in computational scale of digital evolution could induce qualitative effects \citep{moreno2022engineering}, analogously to the renaissance of deep learning with the advent of GPGPU computing \citep{krizhevsky2012imagenet}.

% ELD: TODO: consider cutting this paragraph
Indeed, digital evolution work already commonly marshals substantial parallel and distributed computing  --- in some cases reaching petaflop scale \citep{gilbert2015artificial}.
Methods range from entirely independent evolutionary replicates across compute jobs \citep{dolson2017spatial, hornby2006automated}, to data-parallel fitness evaluation of single individuals over independent test cases using hardware accelerators \citep{harding2007fast_springer, langdon2019continuous}, to application of primary-subordinate/controller-responder parallelism to delegate costly fitness evaluations of single individuals \citep{cantu2001master,miikkulainen2019evolving}.

Fully decentralized, highly-distributed computation is also applied, such as island models \citep{bennett1999building,schulte2010genetic} and mesh-computing approaches \citep{ackley2018digital,moreno2021conduit}.
However, a major barrier to effective applications of the fully-distributed paradigm has been difficulty of observing system state at scale.
In the absence of a global population-level view, the course of evolution becomes much more challenging to study --- undercutting applications of large-scale evolutionary simulation systems as an experimental platform.
Among other instrumentations, including phylogenetic information can help boost observability by providing insight into the mode and tempo of evolution \citep{dolson2020interpreting}.

\subsubsection{Further Applications of Distributed Ancestry Trees}

Replication of digital artifacts pervades computing, and interest in understanding structure of copy trees extends far beyond digital evolution.
Classic examples include the branching reported on the routes through which digital misinformation and computer viruses propagate \citep{friggeri2014rumor,cohen1987computer}.
Studies in this realm have generally relied on centralized tracking, leaving
circumstances where this is not feasible largely underexplored.

Where it has been performed, decentralized copy tracking has proven quite informative.
Work by \cite{libennowell2008tracing} on chain email provides a rare example.
These researchers applied post hoc methods to estimate phylogenies of chain mail messages.
These phylogenies then served as a reference to tune agent-based models, ultimately yielding a remarkable elucidation of email user behavior and underlying social dynamics.
Interestingly, this study's reconstructions were solely enabled by a special peculiarity of the sampled messages: they were email petitions.
Thus, users would append their name to the list before forwarding it on --- a mechanism similar in broad strokes to hereditary stratigraphy.

As an aside, loose parallels between hereditary stratigraphy and visual sedimentation, a dynamic graphic representation that draws on a similar geological metaphor to visualize data streams by progressively stacking, compressing, and then fusing visualized data objects with age, also bear mention \citep{huron2013visual}.

Hereditary stratigraphic techniques enabled new possibilities to delve into hereto cloistered processes through which digital artifacts spread.
Peer-to-peer and federated social networks, which have recently enjoyed substantial upticks in popularity \citep{la2021understanding}, make a prime example.
Within social networks, the structure of share chains is key to understanding, detecting, and mitigating misinformation \citep{kucharski2016study,raponi2022fake} and predatory viral marketing (e.g., spamming and phishing attacks) \citep{guidi2018managing}.
However, existing work relies on the capacity for direct ancestry tracking afforded by monolithic platforms (e.g., Facebook, Twitter, etc.).
Hereditary stratigraphy could enable robust, semi-anonymized extraction of share chain diagnostics within decentralized social networks.

Substantial limitations on uses cases for hereditary stratigraphy should be noted, however.
Annotations predicate influence over the artifact copy process necessary to ensure generational updates.
Additionally, the methodology is susceptible to removal or spoofing of annotation data by antagonistic actors.


==> text/body/methods.tex <==
% \section{Preliminaries} \label{sec:methods}
% This section should introduce the necessary definitions, concepts, and notations that will be used throughout the paper.


==> thm/curbed-recency-proportional-resolution-algo-self-consistency.tex <==
% TODO: missing proof
\begin{theorem}{Curbed Recency-Proportional Resolution Self-Consistency}
\label{thm:curbed-recency-proportional-resolution-algo-self-consistency}

\end{theorem}

\begin{proof}
\label{prf:curbed-recency-proportional-resolution-algo-self-consistency}

\end{proof}


==> thm/curbed-recency-proportional-resolution-algo-space-complexity.tex <==
\begin{theorem}{Curbed Recency-proportional Resolution Space Complexity}
\label{thm:curbed-recency-proportional-resolution-algo-space-complexity}

\end{theorem}

\begin{proof}
\label{prf:curbed-recency-proportional-resolution-algo-space-complexity}

\end{proof}


==> thm/curbed-recency-proportional-resolution-algo-uncertainty-bound.tex <==
\begin{theorem}{Curbed Recency-proportional Resolution Uncertainty Bound}
\label{thm:curbed-recency-proportional-resolution-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:curbed-recency-proportional-resolution-algo-uncertainty-bound}

\end{proof}


==> thm/depth-proportional-resolution-algo-space-complexity.tex <==
\begin{theorem}{Depth-proportional Resolution Space Complexity}
\label{thm:depth-proportional-resolution-algo-space-complexity}

\end{theorem}

\begin{proof}
\label{prf:depth-proportional-resolution-algo-space-complexity}
\end{proof}


==> thm/depth-proportional-resolution-algo-uncertainty-bound.tex <==
\begin{theorem}{Depth-proportional Resolution Uncertainty Bound}
\label{thm:depth-proportional-resolution-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:depth-proportional-resolution-algo-uncertainty-bound}

\end{proof}


==> thm/fixed-resolution-algo-space-complexity.tex <==
\begin{theorem}{Fixed Resolution Space Complexity}
\label{thm:fixed-resolution-algo-space-complexity}

\end{theorem}

\begin{proof}
\label{prf:fixed-resolution-algo-space-complexity}

Given a resolution $a \in \mathbb{N}$, let $f(n) := \frac{n}{a}$. Given $c, k \in \mathbb{N}$, let $P(n) := 0 \le f(n) \le cn \; \forall n \ge k.$

Take $c = a$ and $k = 1$. Then, $P(1): 0 \le \frac{1}{a} \le a,$ so $P(n)$ holds for $n = 1$.

Now, assume that $P(n)$ holds. Then,

\begin{align*}
    P(n + 1) :& \frac{n + 1}{a} &\le (n + 1)a \\
    & \frac{n}{a}  + \frac{1}{a} &\le an + a \\
    & \frac{1}{a} &\le a &&\text{(via $P(n)$)}\\
\end{align*}

And so $P(n) \implies P(n + 1).$ Given that $P(1)$ holds, we can conclude that this algorithm has an $O(n)$ space complexity.

\end{proof}


==> thm/fixed-resolution-algo-uncertainty-bound.tex <==
% TODO: missing proof
\begin{theorem}{Fixed Resolution Uncertainty Bound}
\label{thm:fixed-resolution-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:fixed-resolution-algo-uncertainty-bound}

\end{proof}


==> thm/geom-seq-nth-root-algo-self-consistency.tex <==
% TODO: missing proof
\begin{theorem}{Geometric Sequence $n$th Root Self-Consistency}
\label{thm:geom-seq-nth-root-algo-self-consistency}

\end{theorem}

\begin{proof}
\label{prf:geom-seq-nth-root-algo-self-consistency}

\end{proof}


==> thm/geom-seq-nth-root-algo-space-complexity.tex <==
% TODO: missing proof
\begin{theorem}{Geometric Sequence $n$th Root Space Complexity}
\label{thm:geom-seq-nth-root-algo-space-complexity}
The \gls{extant record size} of the Geometric Sequence $n$th Root Policy Algorithm grows with order $\mathcal{\theta}{(k)}.$

\end{theorem}

\begin{proof}
\label{prf:geom-seq-nth-root-algo-space-complexity}



\end{proof}


==> thm/geom-seq-nth-root-algo-uncertainty-bound.tex <==
% TODO: missing proof
\begin{theorem}{Geometric Sequence $n$th Root Uncertainty Bound}
\label{thm:geom-seq-nth-root-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:geom-seq-nth-root-algo-uncertainty-bound}

\end{proof}


==> thm/recency-proportional-resolution-algo-self-consistency.tex <==
% TODO: missing proof
\begin{theorem}{Recency-proportional Resolution Self-Consistency}
\label{thm:recency-proportional-resolution-algo-self-consistency}

\end{theorem}

\begin{proof}
\label{prf:recency-proportional-resolution-algo-self-consistency}

\end{proof}


==> thm/recency-proportional-resolution-algo-space-complexity.tex <==
\begin{theorem}{Recency-proportional Resolution Space Complexity}
\label{thm:recency-proportional-resolution-algo-space-complexity}

The \gls{extant record size} of the Recency-proportional Resolution Policy Algorithm grows with order $\mathcal{\theta}{(k \log n)}.$

\end{theorem}

\begin{proof}
\label{prf:recency-proportional-resolution-algo-space-complexity}
As per \ref{sec:extant_record_oog}, we will set out to prove that output array of this policy algorithm has an order of growth of $\mathcal{\theta}{(k \log n)},$ where $k$ is a user-provided resolution and $n$ is the number of depositions.

Algorithm \ref{alg:recency-proportional-algo-gen-drop-ranks} determines the array of strata to be dropped at any given time point.
Observe that whenever $2 \mid n$ at least one stratum will be dropped.
More generally, for any positive integer $i \le \log_2 n$, we have that if $2^i \mid n$ then $i$ strata will be dropped. 
Thus, the number of dropped strata is bounded above by $\sum_{i=1}^{\log_2 n} n = n \log_2 n.$
As such, the number of retained strata is bound by $n - n \log_2 n \le \log_2 n$ for all positive $n.$
Given that no strata are dropped when $\frac{n}{2} - 1 < k,$ we observe that the output array of this policy algorithm is bound above by $\mathcal{O}{(k \log n)}.$
Via \ref{sec:extant_record_oog}, we can conclude that this bound is actually $\mathcal{\theta}{(k \log n)}.$
\end{proof}


==> thm/recency-proportional-resolution-algo-uncertainty-bound.tex <==
% TODO: missing proof
\begin{theorem}{Recency-proportional Resolution Uncertainty Bound}
\label{thm:recency-proportional-resolution-algo-uncertainty-bound}

\end{theorem}

\begin{proof}
\label{prf:recency-proportional-resolution-algo-uncertainty-bound}

\end{proof}

